Using Social Information for Flow Allocation in MANETs

Adhoc networks enable communication between distributed, mobile wireless nodes without any supporting infrastructure. In the absence of centralized control, such networks require node interaction, and are inherently based on cooperation between nodes. In this paper, we use social and behavioral trust of nodes to form a flow allocation optimization problem. We initialize trust using information gained from users' social relationships (from social networks) and update the trusts metric over time based on observed node behaviors. We conduct analysis of social trust using real data sets and used it as a parameter for performance evaluation of our frame work in ns-3. Based on our approach we obtain a significant improvement in both detection rate and packet delivery ratio using social trust information when compared to behavioral trust alone. Further, we observe that social trust is critical in the event of mobility and plays a crucial role in bootstrapping the computation of trust.

==> Behavioral_trust.tex <==
\subsection{Calculation of behavioral trust}
\label{behave_trust_12}
Behavioral trust is measured by observing the behavior (actions) of neighbors.  The \emph{observational evidences} $\alpha_o$ (positive evidence) and $\beta_o$ (negative evidence) are collected based on the neighbors actions (behaviors). We illustrate the evidence based behavioral trust calculation by using the following example.

%\subsubsection{Illustrative Example-1: Routing based evidence collection}
\label{routing_t_1}
Let us consider a packet routing scenario in an ad hoc network and let node `$j$' is a target (trustee) node  whose trust is to be calculated. All neighboring nodes within one hop proximity of $j$ can overhear both the incoming packets and the outgoing packets at $j$. The routing table is pre-agreed upon and available at every node and hence a neighboring node of $j$ can easily identify the right destination for each packet. For a fraction of the packets, chosen based on the energy and computation restrictions of the nodes, these neighboring nodes (trustor nodes) can check the destination of each outgoing packet from node $j$ and compare the destination against the routing table available with them.

If the packet advances towards the right destination as per the routing table, then the routing behavior of the trustee node is considered to be correct and trustor can increment the $\alpha_o$ evidence on the trustee. If the packet does not get routed, gets corrupted or modified, or gets routed along an incorrect path, then the experience is recorded as a misbehavior $\beta_o$ evidence on the trustee node. Here we assume that the trustor node can observe both the incoming and outgoing packets at trustee node. %We neglect the effect of packet loss due to interference and fading. %\textit{\textbf{Here we assume that the loss due to fading and interference is minimal. Such issues and packet losses can be accounted into our formulation by extending the behavioral trust model to incorporate packet losses, fading and interference {[ref1, ref2]}.}}

%\subsubsection{Illustrative Example-2: Event monitoring based evidence collection} Let us consider sensor nodes deployed for event monitoring. Every node observes the event and sends observation reports to other nodes. When the event reports are sent, it can be overheard by the one hop neighbour nodes as most of the sensor nodes follow simple broadcast based routing. If the received report readings are not close enough with the reading of own measurement or reading from other overhead nodes, then the observing node can increase the $\beta_o$ on target node, otherwise it can increase the $\alpha_o$ measurement. To be more specific, consider the detection of a moving event (e.g., a moving target such as a vehicle, or a local storm) detection application. The event is defined by a point of maximum intensity (center of event (CoE)) and the event radius $R_e$. In general. events have an intensity profile which decays with distance from the CoE. For a node $j$ at a distance $d(j)$ from the CoE, the measured intensity $I_d(j)$ is given by:
%
%\begin{equation}
%I_d(j)=\frac{cI(t)}{{d(j)}^2}
%\end{equation}
%
%where the event intensity $I(t)$ at time instant $t$, is provided by the application based on known models of the event \cite{event_1}, \cite{event_2}, \cite{event_3} and $c$ is a proportionality constant. Now, a trustor node $i$ at distance $q(i)$ will measure the event as ($I_q(i)$). If the event reports from $j$ match closely enough with the local sensor readings of $i$ after adjusting the distance differences, then the event report by $j$ is considered to be valid by $i$. Hence the $\alpha_o$ evidence can be incremented. Otherwise the $\beta_o$ evidence will be incremented. Here we assume that the loss due to fading and interference is minimal.


The observed evidence values $\alpha_o$ and $\beta_o$ will be used as parameters of a Beta distribution as follows:
\begin{eqnarray}
P(x)=B(\alpha_o, \beta_o, x)=\frac{\Gamma(\alpha_o+\beta_o)}{\Gamma(\alpha_o)\Gamma(\beta_o)}x^{\alpha_o-1}(1-x)^{\beta_o-1}
\label{beta_eqn}
\end{eqnarray}
where $\Gamma(\cdot)$ is the Gamma function. Now the trust opinion will be generated as a triplet $<b, d, u>$, where $b$ stands for node's belief that the neighbor will behave properly in next time, $d$ is the node's disbelief of good behavior and $u$ is the uncertainty of the opinion. The expectation of the beta distribution ( $\alpha_o/(\alpha_o+\beta_o)$), is used to derive $b$ and $d$ and the variance ($Var(t)=\alpha_o\beta_o/(\alpha_o+\beta_o)^2(\alpha_o+\beta_o+1)$), normalized by factor $12$ is used to derive $u$ as shown in Table. \ref{message_table_1}. For brevity we refer to \cite{trust_cal} for detailed calculation of $b$, $d$ and $u$. This belief value $b$ is used as behavioral trust in our work.

We have calculated the behavioral trust based on  Beta distribution using empirical data. A scenario of $40$ nodes deployed over a square region of 100X100 m was assumed.  Ad hoc On-demand Multipath Distance Vector (AOMDV) routing algorithm is used for packet forwarding \cite{marina2002ad}. We calculated the trust based on the routing behavior as described in Section. \ref{routing_t_1}. The behavior was averaged over 100 realizations (see Fig. \ref{behavioral_routing_r1}). We assumed a node has $0.9$ trust factor, another node has $0.8$ trust factor and a third node has $0.7$ trust factor means out of $100$ received packets these nodes do not correctly forward $10$, $20$, $30$ packets uniformly random. Our focus is on testing the effectiveness of our Trust Model, i.e., convergence and accuracy of the trust
calculation in determining the exact value of trust. From Fig. \ref{behavioral_routing_r1} we can see that on an average our approach converge to the correct trust value of these nodes in 14 event observations. In the graph we can see that the initial trust is always less due to uncertainty factor ($u$) which is high in the initial stage. However, as the number of evidences increases the uncertainty slowly reduces and hence the trust value converges to its original value.

\begin{figure}
	\centering
		\includegraphics[width=3in]{figures/behavioural_trust_1.eps}
\caption{Packet routing based behavioral trust calculation}
\label{behavioral_routing_r1}
\end{figure} 

==> Intro_old.tex <==
\begin{abstract}
Mobile ad hoc networks (MANETs) enable communication between distributed, mobile wireless nodes without any supporting infrastructure. In the absence of centralized control, such networks require node coordination in order to establish communication, and are inherently based on trust between nodes to achieve reliable end-to-end communications. In this paper, we address the problem of trustworthy allocation of flows in MANETs using trust as a main factor. To this effect, we develop trust, identity spoofing, and flow diversity metrics and design a flow allocation optimization problem with these metrics. In our trust metrics calculation we initialize trust using information gained from social relationships between users and improve it over time based on observed node behaviors. The identity spoofing metric is calculated based on the trust between nodes, while flow diversity is incorporated to improve robustness to link failures and undetected malicious nodes. We conduct analysis of social trust  using real data sets and used it as a parameter for performance evaluation of our frame work in ns-3. Based on our approach we obtain a significant improvement in both detection rate and packet delivery ratio using social trust information when compared to behavioral trust alone. Further, we observe that social trust is critical in the event of mobility and plays a crucial in bootstrapping the computation of trust.
\end{abstract}
\section{Introduction}
\label{sec:intro}
Mobile Ad hoc NETworks (MANETs) consist of wireless nodes, such as laptops, smart phones, or sensors, operating in the absence of supporting infrastructure. MANETs provide rapid, low-cost deployment, and are therefore attractive for applications such as battlefield communication, enterprise networking, disaster relief, emergency, rescue and providing network access to remote or impoverished communities. Flexibility
of deployment and speed of setup are the key advantages of using MANETs. However, lack of reliability in end-to-end communications has prevented the use of MANETs in many practical applications.

In this paper, we introduce trust metrics as main concept and use them to ensure end-to-end communications and proper operations of MANETs. In our approach trust has two components, {\bf social trust} and {\bf behavioral trust}. Social trust is defined as the strength of the social relationship between the two users. For example, if two users are good friends it is likely that one will assist the other in data flow through his communication device. If we could quantify this social relationship between two users, we could use it to initialize the trust values amongst nodes in a MANET. Such social trust computation is very difficult to quantify, and requires subjective user inputs for each pair of nodes. However, such values can be approximated based on user interactions and profile similarity in social networks.

The other component, {\bf behavioral trust}, is  based on the present and past actions of users. It is measured based on observing and quantifying the actions of the neighbors. Now the combination of social and behavioral trust is used to provide  a unified trust value. This unified trust value can be updated over time based on changes in social relationship between users and observed behavior of other nodes over time.


Apart from the trust relationships, the end-to-end connectivity of MANETs are highly dependent on vulnerability of communication links and quality of the communication channel. To capture these effects, we derive an {\bf identity spoofing} metric to quantify the probability that a malicious node is impersonating a valid node and choose a path accordingly. Trust is the main factor considered in deriving the identity spoofing metric. We also derive a {\bf flow diversity} metric to further ensure reliable end-to-end communications by diversifying the flow amongst multiple reliable paths. These metrics are efficiently combined using distributed optimization with the objective of achieving  reliable end-to-end communication.

The main contributions of this work are as follows:
\begin{enumerate}
\item This paper introduces the idea of incorporating information from social networks and behavioral properties of users to compute `trust' amongst MANET nodes.
\item This paper particularly emphasizes on solving flow allocation problem in MANETs using trust information. We develop unique metrics for identity spoofing and flow diversity. These metrics use social trust information to provide promising end-to-end performance.
\item Sample social trust computations using Inter-profile similarity and Wall post cross-postings of Facebook users have been demonstrated.
\item Extensive performance analysis have been conducted to demonstrate the proposed approach. Results show that we obtain a significant improvement in packet delivery ratio and throughput by using social trust information when compared with behavioral trust alone.
\end{enumerate}

\section{Motivation}
Trustworthy end-to-end communication is an important requirement for practical deployment of MANET. Trust and communication amongst devices takes time to setup and is therefore not easy especially in the mobile scenarios. Vulnerability of communication paths to node misbehavior is another serious consideration preventing widespread deployment of MANETs for enterprise applications. Resource sharing and distributed decision-making enable selfish behaviors (such as overuse of a shared channel or refusing to forward packets by a mobile node to save battery) in MANETs. Furthermore, the lack of centralized authorities imposes additional challenges on detecting misbehavior, thus creating a need for distributed solutions. Distributed trust systems have been proposed to identify nodes exhibiting suspicious behavior. Under trust management systems, each node maintains a trust value for each of its neighbors. Honest behavior, such as correct routing of packets, leads to higher trust values, while suspicious behavior reduces the trust
value.

Implementing trust management systems in MANET presents several key challenges.
\begin{enumerate}
\item First, due to
the distributed and inherently lossy nature of MANET, it may
be difficult to tell the difference between malicious behavior and random failures.
For example, a node may drop packets out of selfishness, or because the connection has timed out.
\item Second, ad hoc networks are highly dynamic, with nodes constantly moving in and out of interaction range.
As a result, there may be little time to develop a trust relationship between nodes based on first-hand
information.
\item Third, while the trustworthiness of a node is only one of the factors influencing node performance.
Device capability, the quality of its communication channels, and its resilience to attack
from external adversaries also affect the reliability of a wireless node.
At present, however, there is no method for combining these factors for distributed decision-making.
\end{enumerate}

In this paper, we envision a scenario where MANETs can be readily deployed, thus reducing the overhead on backbone networks for peer-peer single or multi-hop connections. After rapid deployment, we monitor the performance of each node and route using specific metrics to obtain a full-framework for trusted flow allocation. The latter is achieved by incorporating the metrics for identity spoofing and flow diversity in flow allocation process.

\begin{figure}[t]
	\centering
		\includegraphics[scale=0.35]{figures/manet_block_diagram.eps}
	\caption{Simple diagram of a Mobile Ah-hoc NETwork. Six nodes are connected ad-hoc with each other via WiFi. Social relationships co-exist amongst some users.}
	\label{fig:manet_block_diagram}
\end{figure}

\subsection*{ Relationships Matter}
Wireless communications  and Internet have become commonplace and have completely transformed the social lives of people. Social networking sites such as Facebook (with over 800 million users), Google+, LinkedIn, Orkut (India, Brazil) and Renren (Chinese) have changed the paradigm of adolescent mating rituals, political activism, corporate management styles, classroom teaching and other dimensions of social life. In other words, social networking has made people more social inside the `net', than perhaps outside, in the real-world. This trend is on the increase.

More and more people are using these websites for social interactions and keeping others updated about themselves. Traditionally, people used these `connections' for communicating message from one person to another. People would leverage this social trust on one-another to communicate mails/letters or parcels to another person. In earlier times, if A is going to some city B, his friends will give him any parcels or mails/letters to their acquaintances in that place. Now, social relationships, being formed in online communities, we explore if these online social relationships can similarly help us in better `communication' amongst ourselves.
Basically, we explore a converse question: \textbf{\textit{Can social relationships affect the way wireless nodes interact with each other?}}

Consider the scenario given in Fig~\ref{fig:manet_block_diagram}. The active links between wireless devices are as shown in the figure. The social relationships between users are shown by green connections. It can be observed in this case that B has a good relationship with A and C, but poor relationship with D. Therefore,  D may drop a packet forwarded by B. Thus, poor social trust values are an indicative of `selfish' node behavior and higher social trust values will oblige a node to properly route the packets of another node. Such trust values may be derived from a direct relationship between the users, a relationship with a mutual acquaintance, membership in the same organization, or from online social network data. Unlike behavioral trust, social trust values exist independent of the ad hoc network, and are therefore not sensitive to changes in network topology or communication link failures. These social relationships in fact allow us to compute social trust values which empower MANETs for rapid deployment.

In this paper, we consider a network where ad hoc nodes in MANETs have active relationships. For example, MANET nodes may have cached values of social relationships (off-line), may have access to an online social network like Facebook (online - in a backbone network) or may have access to adhoc-social network (such as Adsocial~\cite{sarigöl09} or MobiSN~\cite{li09mobisn} or others~\cite{gurecki09}).  Such combined networks are under active research consideration these days. CenseMe where mobile phones create mobile sensor networks and share the sensed information in social networks (Facebook) is one architecture in this direction \cite{censeme}.


Use of trust relationships in this combined network addresses first two challenges enumerated earlier. First, based on the behavioral trust on the user, we can determine (probabilistically), whether the packet drop is because of random failure (in case of high trust value), or more probably due to malicious behavior. Secondly, although mobility may obstruct behavioral trust computation, social trust can be calculated based on existing social 	relationships between users and ease trust assessment.

\subsection*{Metrics for Trusted Flow Allocation}
Trust serves as a metric in allocation of flow over a specific path. The traffic may get adversely affected due to vulnerability of the key used for encrypting the communication or the channel may be lossy and disturbed due to mobility or physical parameters. We define two more metrics to account for these factors.

An adversary may attempt to infiltrate the network by impersonating a valid node.  While this infiltration may be prevented by cryptographic mechanisms (i.e., by requiring each node to sign a challenge using a key known only to the claimed owner of the node), in practice MANET are typically deployed without a centralized public key infrastructure.  As a result, nodes rely on distributed, certificate-based methods to validate each other's identities.  {\bf Identity spoofing metrics} describe the confidence that a node $i$ has that node $j$ has the identity it claims, based on the certificates presented by node $j$. We formulate the identity spoofing metric as a function of  combined trust (social and behavioral).

In a dynamic network such as MANET, throughput may also be affected by disruptions caused by link failure or mobility. One approach in mitigating these disruptions is to divide the flows among multiple paths.  This  flow diversity prevents the source-destination connection from being disrupted by the removal of a single path, which may be caused when a relay node moves out of range.  We propose the use of {\bf flow diversity metric} to quantify the level of diversity provided by a given flow.


We use  {\bf trust, identity spoofing,} and {\bf flow diversity} metrics to develop a  distributed flow allocation problem. This is formulated as an optimization framework to maximize the throughput between the source and destination nodes. The capacity of the intermediate links between the source and destination acts as an upper bound on the throughput for a given path.  Maximizing source-destination flow subject to capacity constraints is the goal of classical max-flow/min-cut optimization problems, as well as most widely-used flow control algorithms such as TCP. We devise a multi parameter optimization problem with these constraints. Different factors affecting node performance and flow allocation can be quantified and added to this formulation. This addresses the third challenge enumerated in implementing trust management system in MANETs.


==> Joint_trust_v1.tex <==







%The idea is user pairs with low number of wall posts may be casual acquaintances in Facebook, while user pairs who generated high rates of wall posts may represent close friends.


%Likewise, different wall posting rates may indicate that the relationship between individuals evolve with different patterns. The research studies in show that the high-level interaction group initiates conversation immediately after becoming friends, but their rate of conversation decays over time. On the other hand the low-level interaction group typically takes more than a month to initiate their wall interaction since the time they become friends.


%For this, we calculate the cumulative distribution function (CDF) of the number of wall posts for each user pair. Based on the skewness of the CDF curve we determine the probability of the wall posts exchanges between two pairs. Based on this probability we determine the social trust level. For example if the probability of exchanging $\alpha$ number of wall posts is greater than $\beta$ then we assign the social trust as $\beta$. The value of $\alpha$ is user dependent and measured based on the total number of wall post a particular user exchanges with all users.


\subsection{Calculation of combined trust:}
We use $T_{i,j}(t)$ to denote the unified trust on $j$ by $i$ at time $t$. This value varies from 0 to 1. $S_{i,j}(0)$ is the social trust value and this is used to initialize Trust.

\begin{equation}
T_{i,j}(0)=S_{i,j}(0)
\label{boot_1}
\end{equation}
The trust value is updated based on the following equation:

\begin{equation}
\begin{split}
T_{i,j}(t+1)= &\left (\epsilon - \zeta \hat{u}(\frac{1}{2}- \hat{B}_{i,j}(t) ) \right )\times T_{i,j}(t) \\&+ \left (1-\epsilon \right )\times \hat{B}_{i,j}(t),~0 \le \epsilon,\zeta\le 1	
\label{boot_2}
\end{split}
\end{equation}

where $\hat{B}_{i,j}(t)$ is behavioral trust of $i$ on $j$ at time $t$ and $\hat{u}(t)$ is the step function. As per this update, when the behavioral trust goes below $0.5$, we actually penalize the total trust in the trust update by a factor of $\zeta$. $\epsilon$ denotes the weight we give to current behavior in updating the trust.



When the user updates his social trust values ($S_{i,j}(t)$) (which is not so often updated), trust is recalculated as given below:

\begin{equation}
T_{i,j}(t+1)=  \rho\times T_{i,j}(t) + \left (1-\rho \right )\times S_{i,j}(t),~0 \leq \rho \leq 1
\label{final_trust_so_beh}
\end{equation}
To analyze the bootstrapping of the trust calculation using social networks we synthetically generated features details of users and applied IPS algorithm on the features. The user profiles are text files with the feature details of interests, activities, affiliations, gender. These features follow the vocabulary as described in \cite{felix_ips}. IPS score and Beta distribution are used to calculate social trust as given in \eqref{social_ips_1}. We assume the interaction details are nil at the time $0$. Hence IPS score fully governs the social trust in bootstrapping (i.e., $\eta=0$). This social trust is used in \eqref{boot_1}, \eqref{boot_2} with the $\epsilon$ value of $0.7$, $\zeta$ value of $0.1$. The behavioral trust $\hat{B}_{i,j}(t)$ is calculated using Section. \ref{behave_trust_12}. We assume one node (trustee) has $0.7$ trust value and a trustor wants to estimate that particular node's trust. Both trustee and trustor have social profiles with feature details chosen from a vocabulary set of \cite{felix_ips}. The trust convergence on trustee node by trustor node with this setup is shown in Fig. \ref{fig:social_behavioural_comparison}. We can observe that the trust converges faster when we use both behavioral and social trusts compared to the case where we use behavioral trust alone.
%Social trust is generally used for bootstrapping in the trust calculation. As the time grow generally the behavioral trust will have much impact.


==> Model.tex <==
\section{System Model}
\label{sec:model}
%In this section, we define metrics for flow allocation and state the flow allocation optimization problem, as well as a distributed solution algorithm.
%\begin{enumerate}
%\item The trust values of each user, based on social relationships and observed %\item The probability that the symmetric encryption and authentication keys used by the flow are secure.
%\item The probability that any asymmetric encryption keys belong to the advertised %\item Flow allocation  incorporates \emph{diversity}, so that the communication flows are spread among multiple paths to reduce vulnerability to denial-of-service attacks.
%\end{enumerate}

%\subsection{System Model}
%\label{subsec:comm_model}
We assume a set of users that communicate over a wireless network.  A wireless link $(i,j)$ exists between users $i$ and $j$ if $j$ is
within $i$'s wireless range; let $L$ denote the set of links.  Each link $l \sim (i,j)$ has a nonnegative capacity $c_{l}$.

Two (not necessarily disjoint) subsets $S,D \subseteq V$ of users act as data sources and destinations, respectively.
Each source $s \in S$ sends unicast traffic to a destination, denoted $d_{s} \in D$, with rate $r_{s}$.
When $d_{s}$ is not an immediate neighbor of $s$, $s$ maintains a set of paths, denoted $\mathcal{P}_{s}$, using an ad hoc
routing protocol \cite{jacquet2001optimized, perkins1999ad}.  Each path $\pi \in \mathcal{P}_{s}$ consists of a set of intermediate
links, so that $\pi = \{(s,i_{1}), \ldots, (i_{k}, d_{s})\}$.  Letting $r_{s,\pi}$ denote the rate of traffic from source
$s$ through path $\pi$, flow conservation and capacity requirements imply the following constraints:
\begin{IEEEeqnarray}{rCl}
\sum_{s \in \mathcal{S}}{\sum_{\pi \in l}{r_{s,\pi}}} &\leq& c_{l} \qquad \forall l \in L \\
\sum_{\pi \in \mathcal{P}_{s}}{r_{s, \pi}} &=& r_{s} \qquad \forall s \in S
\end{IEEEeqnarray}
where $\{\pi \in l\}$ denotes the set of paths that include $l \in L$ as an intermediate link.


%\subsection{Social network and user model}
%\label{subsec:social_model}
%A link $(i,j)$ in the social network exists if user $i$ has a trust relationship with user $j$;
%let $E^{\prime}$ denote the set of social network
%links.  Let $t_{ij} \in [0,1]$ denote the trust value of $i$ for $j$, representing $i$'s perceived probability
%that $j$ is trustworthy.

%We assume two types of users in the network, \emph{benign} and \emph{malicious}.
%Benign users who are not source nodes attempt to maximize the global utility by forwarding all packets they receive. Benign users who are also source nodes forward all packets they receive, and attempt to maximize their source rate using any residual capacity.  We assume that benign users have access to cached social network data that is used to compute social trust metrics.
%Benign users who are also source nodes
%attempt to maximize their source rates, while benign non-source nodes attempt to maximize the global utility.
%Malicious users,
%on the other hand, attempt to reduce the throughput of one or more sources.  This can be done when the malicious users lie
%on a source-destination path, and can drop or re-order packets.

\subsection*{Adversary Model}
\label{subsec:adversary}
We assume an adversary with knowledge of the network topology and protocols used by the valid nodes.  The adversary has the ability to join the network and interact with the valid nodes using one or more malicious nodes.  When participating in network protocols, such as routing, the adversary can modify, drop, or re-route packets, and can disobey protocols at other layers, such as medium access.    The malicious nodes may either be fully distributed, or coordinate among themselves, or be controlled by a centralized entity.  Malicious nodes are capable of creating user accounts on social networks, but cannot modify the social network data of valid nodes.   

==> Simulation.tex <==
\section{Simulation Study}
\label{sec:simulation}
In this section, results of simulations conducting the ns-3 network simulator [CITE NS-3] are provided.  The simulation setup is described as follows.

\subsection{Simulation Setup}
\label{subsec:setup}

A network of $20$ nodes, deployed in a static 5x4 grid, was simulated.  A path-loss propagation model with $P_{r} = P_{t}d^{-3}$ was assumed, where $P_{r}$ is the received signal power, $P_{t}$ the transmitted signal power, and $d$ the distance between sender and receiver.  Nodes were assumed to communicate using the 802.11a PHY and MAC protocols, with AODV as the ad hoc routing protocol.  The nodes in the top left and top right acted as sources, while the nodes at the bottom left and bottom right acted as destination.  Each source maintained a flow to each destination.

The following social trust models were considered.  In the first model, users $n_{1}$ and $n_{2}$ [will draw figure for each of these] were assumed to be malicious and dropped all packets forwarded through them.  The remaining users held initial trust values of $0.5$ for $n_{1}$ and $n_{2}$ (corresponding to marginal trust) and $1$ for all other users.  This represents a \emph{known malicious node} scenario.
In the second model, $n_{1}$ and $n_{2}$ were malicious as before, but the remaining nodes had no initial trust values for them; instead, all trust values were initiated to $0.7$.  This represents an \emph{unknown malicious node} scenario.  In the third model, two non-malicious nodes had initial trust values of $0.5$, while each node assigned a trust value of $1$ to the malicious nodes.  This represents an \emph{insider attack} scenario.  For each of these scenarios, data were gathered on the throughput and packet delivery for each source over time, as well as the trust values of the valid and malicious nodes. The results are presented in the following section.

\subsection{Simulation Results}
\label{subsec:sim_results} 


==> Simulation2.tex <==
\section{Simulation Study}
\label{sec:simulation}

In this section, an ns-3 \cite{ns3} evaluation of our proposed flow control approach is described.

\subsection{Simulation Setup}
\label{subsec:simul_setup}

A network of $40$ nodes was simulated, with initial node positions chosen uniformly at random from a rectangular region of area $1500$m x $1500$m.  Static network topologies were considered, as well as a random waypoint mobility model with node speeds varying from 1 m/s to 5 m/s.  A free-space path loss propagation model was assumed, resulting in each node having a radio range of approximately $400$m.  IEEE 802.11a was used at the PHY and MAC layers.

 A subset of five nodes was chosen uniformly at random and designated as malicious nodes.  Upon receiving a packet for forwarding, a malicious node discarded the packet without forwarding with probability $0.5$.  The probability $0.5$ was chosen under the assumption that malicious nodes will sometimes forward packets correctly in order to appear cooperative.  When a node $i$ sent a packet to node $j$ for forwarding and node $j$ failed to forward the packet, node $i$ used this as evidence of malicious behavior and updated node $j$'s trust value accordingly (Eq. [give number]).  Conversely, correct forwarding of packets was used as evidence of good node behavior.  In addition to evidence-based trust, nodes were assumed to have access to an online social network, in which malicious nodes had trust value $0.5$ and valid nodes had trust value $0.9$.

 Four pairs of nodes, designated as $(s_{i}, d_{i})$, $i=1,\ldots, 4$, were chosen at random from the set of non-malicious nodes to act as sources ($s_{i}$) and destinations ($d_{i}$).   Each source $s_{i}$ determined a set of paths to destination $d_{i}$ using a modified version of the Ad hoc On-demand Multipath Distance Vector (AOMDV) routing protocol \cite{marina2002ad}.  The routing protocol was modified to include trust values in route advertisement packets, allowing sources to compute the overall trust of a path.  Based on the gathered route and trust information, each source chose a flow allocation according to \ref{eq:flow_opt}).  Measurements were gathered under three scenarios: in the first, nodes used both social and evidence-based trust values, as in [GIVE EQUATION NUMBER].  In the second, nodes used evidence-based trust alone, while in the third no trust metrics were used.

 \subsection{Simulation Results}
 \label{subsec:results}

 \begin{figure*}[t]
\centering
$\begin{array}{ccc}
\includegraphics[width=2in]{figures/Figure_3a_PDR_static.eps} &
\includegraphics[width=2in]{figures/Figure_3b_throughput_static.eps} &
\includegraphics[width=2in]{figures/Figure_3e_detection_static.eps}\\
(a) & (b) & (c)\\
\includegraphics[width=2in]{figures/Figure_3c_PDR_mobility.eps} &
\includegraphics[width=2in]{figures/Figure_3d_throughput_mobility.eps} &
\includegraphics[width=2in]{figures/Figure_3f_detection_mobility.eps} \\
(d) & (e) & (f)
\end{array}$
%\includegraphics[width=3.5in]{Simulation_one_few_trials.eps}
\caption{Performance of ad hoc networks under different mobility and trust models. (a) In a static network, incorporating social trust increases the packet delivery ratio compared to behavioral trust. (b) This increase in delivery ratio results in an increase in achieved throughput.  (c) Social trust also increases the probability of detecting a malicious user and routing traffic around that user. (d), (e) In a network of mobile users, there is a larger improvement in delivery ratio and throughput from social trust. (f) Probability of detection in a mobile environment.}
\label{fig:performance}
\end{figure*}

Figures \ref{fig:performance}a and \ref{fig:performance}b show the average packet delivery ratio and throughput, respectively, over time in the case of a static network.
Using social trust, the sources are able to identify and avoid routes containing malicious nodes, resulting in high throughput and delivery ratio.
When only evidence-based trust is used, however, nodes are unable to accumulate enough evidence to avoid malicious nodes.
As a result, the performance of evidence-based trust is comparable to that when no trust metrics are used.

The impact of malicious users is exacerbated when nodes are mobile.  Due to mobility, each node will have limited time to observe its neighbors, and hence cannot gather sufficient evidence to evaluate that node's reliability.  This results in a further reduction in packet delivery ratio (Figure \ref{fig:performance}d) and throughput (Figure \ref{fig:performance}e).  Since the social trust values are independent of the network topology, incorporating social trust reduces the level of evidence needed to identify malicious nodes, making the trust management scheme robust to topology changes.
\begin{figure}[h]
\centering
\includegraphics[width=2.5in]{figures/Figure_5_mobility.eps}
\caption{Effect of mobility on packet delivery ratio using different trust metrics.}
\label{fig:mobility}
\end{figure}

The impact of mobility is further illustrated in Figure \ref{fig:mobility}.  In all three trust management scenarios (social and evidence-based trust, evidence-based trust alone, and no trust management), there is a decrease in packet delivery ratio as node speed increases.  This is because routes become inactive at a higher rate, leading to losses when packets are sent over links that no longer exist.  Furthermore, when new routes are selected in response to topology changes, they may include malicious nodes.  Under the social trust-based method, these malicious nodes are detected faster, and hence flows are not allocated along routes containing malicious nodes.

\begin{figure}[h]
\centering
\includegraphics[width=2.5in]{figures/Figure_7_malicious.eps}
\caption{Performance degradation as number of malicious users increases.}
\label{fig:malicious}
\end{figure}

The effect of malicious nodes is more pronounced as the number of malicious nodes in the system increases (Figure \ref{fig:malicious}).  When only behavioral trust is used, gathering enough evidence to avoid all malicious nodes becomes increasingly difficult.  Using social trust mitigates this effect, until the number of malicious nodes increases to the point where they cannot be avoided in routing.

\begin{figure}[h]
\centering
\includegraphics[width=2.5in]{figures/Figure_8_threshold.eps}
\caption{Effect of trust threshold on performance.}
\label{fig:threshold}
\end{figure}

In addition to the number of malicious nodes, network performance is affected by the trust threshold, $\tau_{T}$ (Figure \ref{fig:threshold}).  When the threshold is low, any route, even one containing untrustworthy nodes, can be used for packet delivery, resulting in malicious behavior and packet drops.  As the threshold increases, the delivery ratio improves; however, if the threshold is too high, then no nodes will meet the threshold, and hence no paths can form.

%e.	This lack of evidence is further reflected in Figure 3c, which shows the probability that a source node's route does not contain any malicious users
%f.	Detection of malicious users is much slower under the evidence-based schemes than when social trust is 

==> Spoofing.tex <==
\subsection{Verifying user identities}
\label{subsec:asymmetric}
%The users of the network may employ cryptography in order to authenticate each other and check the integrity of certain packets.
The use of social trust data by node i to determine the trustworthiness of node j can be thwarted if a selfish or malicious
user masquerades as a user trusted by i. This can be incorporated into trust metrics by asking a set of nodes, denoted $R(j)$,
 to vouch for j's true identity, as described by the following metric.

%User $i$'s level of trust in $PK_{j}$, denoted $SM(i,j)$ represents the belief that $PK_{j}$ was actually created by user $j$ instead of a malicious user spoofing the identity of $j$.  It is defined as a function of the trust values of the nodes in $R_{j}$, as follows:
\begin{definition}
\label{def:asymmetric_metric}
The \emph{identity spoofing metric} $ISM(i,j)$ for link $(i,j)$ is defined to be the probability that
at least one of the users in $R_{j}$ is valid, given by
\begin{equation}
\label{eq:asymmetric_metric}
ISM(i,j) = 1 - \prod_{r \in R_{j}}{(1 - T_{i,r}ISM(i,r))}
\end{equation}
\end{definition}
where $T_{i,r}$ is the combined trust factor of $i$ on $r$ (combination of social and behavioral trust), and $ISM(i,r)$ is the trust of $i$ on $r$'s identity. It is assumed that $i$ has independently verified the identity of at least one user, $j$, resulting in $ISM(i,j) = 1$. This independence assumption is required to maintain a basic level of trust on each other's identity which is then propagated using combined trust metric ($T_{i,r}$). The values of $ISM(i,j^{\prime})$, for all $j^{\prime} \in V$, can then be computed using the fully-trusted users as a starting point.
 In (\ref{eq:asymmetric_metric}), $T_{i,r}ISM(i,r)$ is the probability that a node $r$'s claim of node $j$'s identity is trustworthy, equal to the probability that $r$ is a trustworthy user ($T_{i,r}$) times the probability that $r$'s identity is correct ($ISM(i,r)$). We observe that, if one of the nodes in $R_{j}$ is fully trusted ($T_{i,r} = ISM(i,r) = 1$), then $ISM(i,j)=1$ in (\ref{eq:asymmetric_metric}).
